End-to-End Neural Entity Linking

Entity Linking (EL) is an essential task for semantic text understanding and information extraction. Popular methods separately address the Mention Detection (MD) and Entity Disambiguation (ED) stages of EL, without leveraging their mutual dependency. We here propose the first neural end-to-end EL system that jointly discovers and links entities in a text document. The main idea is to consider all possible spans as potential mentions and learn contextual similarity scores over their entity candidates that are useful for both MD and ED decisions. Key components are context-aware mention embeddings, entity embeddings and a probabilistic mention - entity map, without demanding other engineered features. Empirically, we show that our end-to-end method significantly outperforms popular systems on the Gerbil platform when enough training data is available. Conversely, if testing datasets follow different annotation conventions compared to the training set (e.g. queries/ tweets vs news documents), our ED model coupled with a traditional NER system offers the best or second best EL accuracy.

==> ablation.tex <==

%
%
%\paragraph{Ablation Study.}
%Ablation studies are conducted and shown in Tables \hi{CITE}. We can see that bi-LSTMs for context vectors are a key component of our system, as removing them would result in a significant drop in performance. In addition, we observe that character embeddings are important for finding lexical patterns in text. Regarding the "soft head" mechanism for mention embeddings, it does not improve our results on AIDA datasets, but it is useful for other test datasets.
%
%
%
%
%Here we evaluate the contribution of each component of our neural network to the final result. We also evaluate alternative architectures. For each different architecture we conduct \textbf{three experiments} and we report the mean and the confidence interval for confidence 90\% of the \textbf{F1 EL} scores.
%
%\begin{enumerate}
%\item \textbf{Base Model}: Our base model (named \textit{model} in the results tables), as explained before, does not use long range attention and global disambiguation; also it uses simple projections instead of deep FFNNs (for $\text{FFNN}_1$ and $\text{FFNN}_2$) and it does not use the head attention mechanism.
%The size of the character embeddings is 50, the character LSTMs have hidden dimensions of 50, the contextual LSTMs have hidden size of 150.\\
%
%
%\item \textbf{Double LSTMs hidden size}: We now double the size of the character embeddings to 100, the character LSTMs to 100, the contextual LSTMs to 300. We observe a slight improvement.
%
%\item \textbf{+soft mention head on word emb}: Here we have the Base Model plus the soft mention head on word+char embeddings (formula \ref{soft_mention_head}: $\hat{x}^m = \sum_{k=q}^r a^m_{k} \cdot v_k $). We have significant improvement on both dev and test sets.
%
%\item \textbf{+soft mention head on ctxlstm emb}: Similar to the previous experiment, but now the attention is over the contextual Bi-LSTM embedding vectors. Now, formula \ref{soft_mention_head} becomes: $\hat{x}^m = \sum_{k=q}^r a^m_{k} \cdot x_k $.
%We have no improvement at all in comparison with the Base Model.
%
%\item \textbf{-char emb}: From the Base Model we remove completely the character embeddings. Only a very small decrease in performance is observed.
%
%\item \textbf{Global -lstm similarity score}: Our Global Model (as shown in figure \ref{fig:full_model}) uses the 1) $\text{log}p(e|m)$ 2) the \textit{lstm similarity score} 3) the \textit{long range attention score} 4) and the \textit{global voting score}. In this experiment we remove completely the \textit{lstm similarity score}. The performance decreases to less than half, hence we deduce that this is the most crucial component of our neural network.
%
%\item \textbf{-ctxlstm}: Now we remove only the bidirectional context-LSTM which means that we continue to calculate the \textit{similarity scores} but now the mention embedding is computed directly from the word-character embeddings $v_k$ instead of $x_k$. Formula \ref{formula_mention_emb} becomes $g^{m} = [v_q; v_r]$. The performance drop is more than 10\%, verifying the crucial role of the context-lstm component.
%
%\item \textbf{-ctxlstm +soft mention head on word emb}: Similar to the previous experiment, however, now we also use the soft mention head mechanism. Formula \ref{formula_mention_emb} becomes $g^{m} = [v_q; v_r; \hat{v}^m]$. Here we observe that the head mechanism offers significant improvement (1.7\%), whereas in the Base Model (experiments 1 and 3) the improvement is lower (0.6\%). However, this is expected, as in the Base Model we use the context aware word embeddings $x_k$ which already capture the context -- hence the words from inside the mention span; whereas in this experiment, the only way to capture the inside words of a mention span (with length more than two words) is only through the head mechanism. 
%
%\item \textbf{Base Model -$\text{log}\mathbf{p(e|m)}$}: From the Base Model we omit the $\text{log}p(e|m)$ (hence we make predictions solely from the lstm similarity scores). As expected, the performance decreases.
%
%\item \textbf{Global Model -$\text{log}\mathbf{p(e|m)}$}: From the Global Model (model+att+global) we omit the $\text{log}p(e|m)$. As expected, the performance decreases. This and the previous experiment show that the $\text{log}p(e|m)$ information is important and cannot be substituted by the information provided by the other components even for the global model. % TODO!! comparison with the full model later
%
%\item \textbf{+$\text{FFNN}_2$ (dropout)}: In this experiment we use a $\text{FFNN}_2$ with one hidden layer with 100 units. We also use dropout for regularization (2 $\rightarrow$ 100 $\rightarrow$ ReLU $\rightarrow$ Dropout $\rightarrow$ 1). Here we observe a slight decrease on the dev set but an increase on the test set. However, from many other experiments that we have conducted and are not reported here we conclude that its usage is not beneficial. Therefore, in the results reported in the previous chapter none of the models used it (they used simple projections).
%
%\item \textbf{Attention Model (model+att)}: This is the Base Model plus Long Range Context Attention.
%
%\item \textbf{Global Model}: This is the model depicted in figure \ref{fig:model} and has the name \textbf{model+att+global} in  table~\ref{tab:ablation}

%%\item \textbf{+$\text{FFNN}_1$}: Table~\ref{tab:14}. The $\text{FFNN}_1$ takes as input the mention embeddings $x^m$ and outputs 300-dimensional vectors. In our Base Model we use simple projection (no hidden layers, i.e. $Wx^m + b$). However, the mention embeddings $x^m$ have high dimensionality (usually 600 or more) and thus $W$ introduces a lot of new variables. With this line of experiments we test if by reducing this number of variables -- by using a narrow FFNN (like an autoencoder) -- we can observe any performance gain. Specifically, we test the following: a) $x^m \rightarrow 3 \rightarrow 300$ b) $x^m \rightarrow 30 \rightarrow 300$ c) $x^m \rightarrow 100 \rightarrow 300$. All of them perform worse than the Base Model which in essence is equivalent to $x^m \rightarrow 300$. The experiments that have \textit{Frobenius} in their name use the Frobenius regularization (explained in the next bullet) in comparison with the rest that use dropout.
%%%\begin{enumerate}[label*=\arabic*.]
%
%
%%\item \textbf{FFNN frobenius norm bound}: Table~\ref{tab:15}. Until now, the only regularization that we apply to our neural network is dropout. In the three FFNNs we apply dropout on the hidden layers. Thus a FFNN with one hidden layer can be written as input $\rightarrow W_h x+b_h \rightarrow \text{ReLU} \rightarrow \text{Dropout} \rightarrow W_o x + b_o $. Now, we will replace the dropout regularization with frobenius norm upper bound. Specifically, we impose the restrictions: $\norm{W_h}_F \leq c$, $\norm{b_h}_F \leq c$, $\norm{W_o}_F \leq c$, $\norm{b_o}_F \leq c$. The experiments that include \textit{only hidden layer} in their name impose this restriction only to $W_h$ and $b_h$ and not to the output layer. All the experiments use the Frobenius norm bound and we observe they perform worse than the corresponding experiments without it.
%
%
%
%%
%%\begin{table*}[h!]
%%  \begin{center}
%%    \label{tab:datasets}
%%    \begin{tabular}{l| c| c| c| c}    % S
%%      \textbf{Model description} & \rot{\textbf{\begin{tabular}{@{}l@{}}AIDA Dev\\Micro F1 \%\end{tabular}}} & \rot{\textbf{\begin{tabular}{@{}l@{}}AIDA Test\\Micro F1 \%\end{tabular}}} & \rot{\textbf{\begin{tabular}{@{}l@{}}AIDA Dev\\Macro F1 \%\end{tabular}}} & \rot{\textbf{\begin{tabular}{@{}l@{}}AIDA Test\\Macro F1 \%\end{tabular}}}\\
%%      \hline    
%%    \begin{tabular}{@{}l@{}}Base Model+$\text{FFNN}_1$ \\$x^m \rightarrow 3 \rightarrow 300$ \end{tabular}					&  	$77.2 \pm 3.6$		& 	$73.6 \pm 2.9$	&   $74.3 \pm 3.5$ 	&	$74.8 \pm 2.4$	\\  
%%    \begin{tabular}{@{}l@{}}Base Model+$\text{FFNN}_1$ \\$x^m \rightarrow 30 \rightarrow 300$ \end{tabular}					&  	$87.1 \pm 0.7$		& 	$79.8 \pm 0.7$	&   $84.8 \pm 0.7$ 	&	$81.1 \pm 1.1$ 	\\
%%    \begin{tabular}{@{}l@{}}Base Model+$\text{FFNN}_1$ \\$x^m \rightarrow 100 \rightarrow 300$ \end{tabular}					&  	$88.1 \pm 0.9$		& 	$80.1 \pm 0.9$	&   $85.7 \pm 1.3$ 	&	$81.5 \pm 0.6$	\\
%%    \begin{tabular}{@{}l@{}}Base Model+$\text{FFNN}_1$ \\$x^m \rightarrow 30 \rightarrow 300$ (Frobenius) \end{tabular}					&  	$84.5 \pm 0.1$		& 	$78.4 \pm 0.5$	&   $81.7 \pm 0.8$ 	&	$78.9 \pm 0.7$	\\
%%    \begin{tabular}{@{}l@{}}Base Model+$\text{FFNN}_1$ \\$x^m \rightarrow 100 \rightarrow 300$ (Frobenius) \end{tabular}					&  	$83.3 \pm 1.4$		& 	$77.3 \pm 0.3$	&   $80.6 \pm 1.2$ 	&	$77.7 \pm 1.0$	\\
%%    \end{tabular}
%%    \caption {Experiment 14: (+$\text{FFNN}_1$). Mean value and 90\% confidence intervals for EL local scores.}
%%    \label{tab:14}
%%  \end{center}
%%\end{table*}
%
%%
%%\begin{table*}[h!]
%%  \begin{center}
%%    \label{tab:datasets}
%%    \begin{tabular}{l| c| c| c| c| c}    % S
%%      \textbf{Model description} & \rot{\textbf{\begin{tabular}{@{}l@{}}AIDA Dev\\Micro F1 \%\end{tabular}}} & \rot{\textbf{\begin{tabular}{@{}l@{}}AIDA Test\\Micro F1 \%\end{tabular}}} & \rot{\textbf{\begin{tabular}{@{}l@{}}AIDA Dev\\Macro F1 \%\end{tabular}}} & \rot{\textbf{\begin{tabular}{@{}l@{}}AIDA Test\\Macro F1 \%\end{tabular}}} & \rot{\textbf{\begin{tabular}{@{}l@{}}AIDA Test\\Micro F1 \%\\ $\Delta$ from table \ref{tab:ablations_main}\end{tabular}}}\\
%%      \hline    
%%    Base Model	($c=1$) 			&  	$83.8 \pm 2.1$		& 	$77.7 \pm 1.6$	&   $80.5 \pm 2$ 	&	$78.3 \pm 1.5$	& $-2.5$\\  
%%    Base Model	($c=3$) 			&  	$86.7 \pm 1.5$		& 	$79.6 \pm 2.1$	&   $84.6 \pm 2.3$ 	&	$80.9 \pm 1.9$	& $-0.6$\\
%%    Base Model	($c=6$) 			&  	$87.4 \pm 1.0$		& 	$79.3 \pm 1.7$	&   $85.1 \pm 1.3$ 	&	$80.6 \pm 2.1$	& $-0.9$\\
%%    Base Model	($c=9$) 			&  	$88.4 \pm 0.8$		& 	$80.4 \pm 0.3$	&   $86.5 \pm 1.2$ 	&	$81.8 \pm 0.4$	& $+0.2$\\
%%    Base Model	($c=1$, hidden only) 			&  	$87.9 \pm 0.1$		& 	$80.0 \pm 1.0$	&   $85.7 \pm 0.3$ 	&	$81.1 \pm 0.1$	& $-0.2$\\
%%    +$\text{FFNN}_2$ ($c=1$)			&  	$81.5 \pm 0.6$		& 	$77.2 \pm 1.2$	&   $78.8 \pm 1.2$ 	&	$76.9 \pm 2.2$  & 	$-3.8$\\
%%    Global Model	($c=1$)				&  	$85.3 \pm 0.2$		& 	$79.9 \pm 0.3$	&   $82.4 \pm 0.4$ 	&	$79.6 \pm 0.4$	& $-1.9$\\
%%    \begin{tabular}{@{}l@{}}Global Model+$\text{FFNN}_2$\\$+\text{FFNN}_3$ ($c=1$)\end{tabular}					&  	$82.6 \pm 0.8$		& 	$79.9 \pm 0.8$	&   $79.7 \pm 1.6$ 	&	$78.8 \pm 0.7$	& $-1.9$\\
%%    \end{tabular}
%%    \caption{Experiment 15: FFNN frobenius norm bound. Mean value and 90\% confidence intervals for EL local scores.}
%%    \label{tab:15}
%%  \end{center}
%%\end{table*}
%
%
%
%%\item \textbf{Global voting alternatives}: Table~\ref{tab:16}. The global disambiguation of the Global Model is described in paragraph \ref{paragraph_global_disambiguation}. One alternative that we test is to calculate the loss in only one point (\textit{one-loss} model). Specifically, the formula \ref{eq:global_loss} now becomes:  
%%\begin{align*} 
%%\theta^* = \arg\min_{\theta} \sum_{d \in D} \sum_{m \in M} \sum_{e \in C(m)} V(\Phi_{\theta}(e,m))
%%\end{align*}
%%A second alternative is to consider a different set of voters for the global disambiguation. Specifically, we modify the formula \ref{global_voters} to: 
%%\begin{align*}
%%V_{\mathit{set}}^{m_i, e_j} &= \{\langle e_j, e \rangle | m \in M\setminus \{m_i\} \land e \in C(m)\}\\
%%G(e_j, m) &= \frac{1}{k} \sum\limits_{x \in topk(V_{\mathit{set}}^{m_i, e_j}) \land x > 0} x\\
%%\end{align*}
%%
%%\begin{table*}[h!]
%%  \begin{center}
%%    \label{tab:datasets}
%%    \begin{tabular}{l| c| c| c| c}    % S
%%      \textbf{Model description} & \rot{\textbf{\begin{tabular}{@{}l@{}}AIDA Dev\\Micro F1 \%\end{tabular}}} & \rot{\textbf{\begin{tabular}{@{}l@{}}AIDA Test\\Micro F1 \%\end{tabular}}} & \rot{\textbf{\begin{tabular}{@{}l@{}}AIDA Dev\\Macro F1 \%\end{tabular}}} & \rot{\textbf{\begin{tabular}{@{}l@{}}AIDA Test\\Macro F1 \%\end{tabular}}}\\
%%      \hline     
%%    Global Model	& 	$89.4 \pm 0.4$ 		&   $81.8 \pm 0.4$	& 	$87.5 \pm 0.2$	&   $83.1 \pm 0.3$ 				\\
%%    Global Model one-loss 	&  	$89.2 \pm 0.2$		& 	$81.3 \pm 0.4$	&   $87.2 \pm 0.3$ 	&	$82.2 \pm 0.6$	\\ 
%%    Global Model topk one-loss 	&  	$88.4 \pm 0.7$		& 	$81.4 \pm 0.6$	&   $87.0 \pm 1.1$ 	&	$82.6 \pm 0.8$	\\
%%    \end{tabular}
%%    \caption{Experiment 16: Global Disambiguation alternatives. Mean value and 90\% confidence intervals for EL local scores.}
%%    \label{tab:16}
%%  \end{center}
%%\end{table*}

%\end{enumerate}



%
%
%\begin{table*}[h!]
%%\begin{adjustwidth}{-2.5cm}{}
%\begin{minipage}{\textwidth}
%  \begin{center}
%    \label{tab:ablations_main}
%    \begin{tabular}{l| c| c| c| c}    % S
%      %\textbf{Model description} & \rot{\textbf{AIDA Dev Micro F1 \%}} & \rot{\textbf{AIDA Test Micro F1 \%}} & \rot{\textbf{AIDA Dev Macro F1 \%}} & \rot{\textbf{AIDA Test Macro F1 \%}}\\
%      \textbf{Model description} & \rot{\textbf{\begin{tabular}{@{}l@{}}AIDA Dev\\Micro F1 \%\end{tabular}}} & \rot{\textbf{\begin{tabular}{@{}l@{}}AIDA Test\\Micro F1 \%\end{tabular}}} & \rot{\textbf{\begin{tabular}{@{}l@{}}AIDA Dev\\Macro F1 \%\end{tabular}}} & \rot{\textbf{\begin{tabular}{@{}l@{}}AIDA Test\\Macro F1 \%\end{tabular}}}\\
%      \hline    
%      1. Base Model 					&  	$88.4 \pm 0.2$		& 	$80.2 \pm 0.5$	&    $86.3 \pm 0.2$	&	$81.6 \pm 0.5$	\\
%      \begin{tabular}{@{}l@{}}2. Double LSTMs hidden size\\	\end{tabular}				& 	$88.5 \pm 0.3$ 		&   $80.3 \pm 1.0$	& 	$86.7 \pm 0.5$	&   $82.2 \pm 0.8$ 	\\
%      \begin{tabular}{@{}l@{}}3. +soft mention head\\ on word emb\end{tabular}			 	& 	$89.1 \pm 0.3$ 		&   $81.3 \pm 0.3$	& 	$87.4 \pm 0.2$	&   $82.1 \pm 1.1$ 	\\
%      \begin{tabular}{@{}l@{}}4. +soft mention head\\ on ctxlstm emb\end{tabular}					& 	$88.3 \pm 0.6$ 		&   $80.2 \pm 0.7$	& 	$86.3 \pm 1.3$	&   $81.8 \pm 0.4$		\\
%      5. -char emb (6 experiments)	& 	$88.3 \pm 0.3$ 		&   $80.3 \pm 0.4$	& 	$86.0 \pm 0.3$	&   $81.3 \pm 0.3$ 				\\
%      6. Global -lstm similarity score	& 	$43.9 \pm 0.3$ 		&   $46.2 \pm 0.8$	& 	$40.1 \pm 0.4$	&   $44.3 \pm 2.3$ 				\\
%      7. -ctxlstm	& 	$78.7 \pm 0.2$ 		&   $72.5 \pm 0.6$	& 	$74.7 \pm 0.2$	&   $72.8 \pm 1.1$ 				\\
%      \begin{tabular}{@{}l@{}}8. -ctxlstm +soft mention head\\on word emb\end{tabular}	& 	$80.4 \pm 1.3$ 		&   $73.2 \pm 1.2$	& 	$76.9 \pm 1.2$	&   $73.7 \pm 1.0$ 				\\
%      9. Base Model -$\text{log}p(e|m)$	& 	$87.4 \pm 0.3$ 		&   $79.0 \pm 1.9$	& 	$76.9 \pm 1.2$	&   $73.7 \pm 1.0$ 				\\
%      10. Global Model -$\text{log}p(e|m)$	& 	$88.0 \pm 0.3$ 		&   $79.3 \pm 2.7$	& 	$86.2 \pm 0.3$	&   $80.9 \pm 1.4$ 				\\
%      11. +$\text{FFNN}_2$ (dropout)	& 	$87.8 \pm 0.3$ 		&   $81.0 \pm 0.4$	& 	$85.7 \pm 0.7$	&   $82.0 \pm 0.3$ 				\\
%      12. Attention Model (model+att)	& 	$88.9 \pm 0.2$ 		&   $81.1 \pm 1.2$	& 	$86.6 \pm 0.8$	&   $82.0 \pm 1.3$ 				\\
%      13. Global Model	& 	$89.4 \pm 0.4$ 		&   $81.8 \pm 0.4$	& 	$87.5 \pm 0.2$	&   $83.1 \pm 0.3$ 				\\
%    \end{tabular}
%    \caption{Alternative Architectures. Mean value and 90\% confidence intervals for EL local scores.}  
%  \end{center}
%\end{minipage}
%\end{table*}



